Do Large Language Models Understand Conversational Implicature -- A case study with a chinese sitcom

Understanding the non-literal meaning of an utterance is critical for large language models (LLMs) to become human-like social communicators. In this work, we introduce SwordsmanImp, the first Chinese multi-turn-dialogue-based dataset aimed at conversational implicature, sourced from dialogues in the Chinese sitcom $\textit{My Own Swordsman}$. It includes 200 carefully handcrafted questions, all annotated on which Gricean maxims have been violated. We test eight close-source and open-source LLMs under two tasks: a multiple-choice question task and an implicature explanation task. Our results show that GPT-4 attains human-level accuracy (94%) on multiple-choice questions. CausalLM demonstrates a 78.5% accuracy following GPT-4. Other models, including GPT-3.5 and several open-source models, demonstrate a lower accuracy ranging from 20% to 60% on multiple-choice questions. Human raters were asked to rate the explanation of the implicatures generated by LLMs on their reasonability, logic and fluency. While all models generate largely fluent and self-consistent text, their explanations score low on reasonability except for GPT-4, suggesting that most LLMs cannot produce satisfactory explanations of the implicatures in the conversation. Moreover, we find LLMs' performance does not vary significantly by Gricean maxims, suggesting that LLMs do not seem to process implicatures derived from different maxims differently. Our data and code are available at https://github.com/sjtu-compling/llm-pragmatics.

==> related_work.tex <==
%%%Recent large language models (LLMs), such as GPT-4, have achieved significant accomplishments in understanding and generating natural language.\citep{bubeck2023sparks}
\section{Related Work}\label{sec:related}

\begin{table*}[t]
\small
\centering
    \begin{adjustbox}{max width=\textwidth}
        \begin{tblr}{Q[l, m]Q[l, m]Q[l, m]Q[c, m]Q[l, m]}
        \toprule
            Dataset         &        Task        &     Context       &         Manually        &   Language \\
        \midrule
            CoQa \citep{reddy2019coqa} & conversational QA & Paragraph & \tick & English \\
            Narrative-QA \citep{kocisky-etal-2018-narrativeqa} & Reading comprehension & Documents & \tick & English \\
            DREAM \citep{sun-etal-2019-dream} & QA & Free-form, multi-turn dialogue & \tick & English \\
            MuTual \citep{cui-etal-2020-mutual} & Next utterance prediction & Free-form, multi-turn dialogue & \tick & English \\
            GRICE \citep{zheng2021grice} & Gricean Implicature Recovery, QA & Fixed form, multi-turn dialogue & \fork & English \\
            PragMega \citep{floyd2023pragmega} & ToM QA & Paragraph & \tick & English \\
            LUDWIG \citep{ruis2022large} & Implicature QA & Single-turn dialogue & \tick & English \\
             Douban \citep{wu-etal-2017-sequential} & Next utterance prediction & Free-form multi-turn dialogue & \fork & Chinese \\
        \midrule
            SwordsmanImp (This work) & Gricean Implicature QA & Free-form, multi-turn dialogue & \tick & Chinese \\
        \bottomrule
        \end{tblr}
    \end{adjustbox}
\label{tab:comparison:datasets}
\caption{Comparing our datasets and the existing datasets. ``Manually" indicates whether the questions or answers are written partly or entirely by human.}
\end{table*}

% \orange{The related work section should be organized around the gaps in previous literature, in addition to what has been done in the field, with the following structure: previous work 1, gap 1; previous work 2, gap 2; .... The first gap could be in pragmatic reasoning studies, and our work fills this gap. The second gap could be in Chinese datasets, and our work fill the gap too... }

Understanding non-literal meanings has long been considered a difficult task for language models. Previous studies have explored the capabilities of language models in recognizing metaphors \citep{wachowiak2023does,neidlein2020analysis}, humor \citep{hessel2022androids,jentzsch2023chatgpt,chen2023can} and social commonsense \citep{sap-etal-2019-social}. Broad-scale datasets aimed at pragmatic reasoning collect data mainly through crowdsourcing or crawling from the internet \citep{reddy2019coqa, kocisky-etal-2018-narrativeqa}. Some others transform the existing tests for humans to train and evaluate language models \citep{cui-etal-2020-mutual, sun-etal-2019-dream}. 
While the above-mentioned datasets have comprehensive coverage for pragmatic understanding, they are not ideal resources for evaluation of a specific type of pragmatic knowledge, that is, conversational implicatures derived by violation of the Gricean maxims.
% The pragmatic knowledge included in these large-scale datasets is too comprehensive to focus on a specific aspect. 
In our work, we craft our dataset manually to make sure that each implicature can be classified to one or more Gricean maxims. This enables us to perform a fine-grained analysis of LLMs' understanding of this particular pragmatic inference.
% It also allows for comparison with human performance on similar tasks to better understand the underlying process of LLMs' pragmatic reasoning. 

Previous attempts in evaluating LLMs' pragmatic understanding guided by the Gricean maxims or cooperative principles do not have multi-turn dialogues from real-world situations. 
% have achieved either linguistically-oriented insights or multi-turn dialogues as context, but never both. 
Formalized under the theory of cooperative principles \citep{grice1975logic}, \citet{zheng2021grice} automatically generated their dataset GRICE through a set of well-defined grammar rules. 
% Each entry in their dataset is generated through fixed syntactic structures. 
This grammar-based method ensures a good control for the pragmatic cues to be aligned with the Gricean maxims. However, dialogues with fixed syntactic structures hardly represent the complexity of conversation in daily communication. While PragMega~\citep{floyd2023pragmega} includes more contextual information and varied forms of dialogues, it includes Gricean implicature as a whole type of questions without discussing the differences between maxims. Moreover, it provides context through a paragraph of scenario description, decreasing the difficulty in decoding situational context from the dialogues, which is more common in human conversation.
%includes Gricean implicature as one of the seven phenomena and provides a rich context for each question, context information is narrated through paragraphs preceding the questions.
% This eliminates the difficulty of understanding the situation from dialogues, a process that happens commonly in human conversations. 
In this study, we fill the gap by providing the multi-turn dialogue directly to the model.
% in the previous research of pragmatic reasoning by establishing a conversational dataset with fine-grained annotation on the Gricean maxims violated in the target sentences appearing at the end of the dialogues that provide contextual information. 

%Language differences should also influence LLMs' dialogue understanding.\orange{This does not sound right. Change to something like: 
% It has also been shown that models' performance varies from one language to another. 
Last but not least, there is a scarcity in Chinese evaluation resources for pragmatic inferences. Previous large-scale conversational datasets in Chinese include Sina Weibo \citep{shang-etal-2015-neural}, Douban conversational corpus \citep{wu-etal-2017-sequential} and E-commerce Dialogue corpus \citep{zhang-etal-2018-modeling}. However, all of them are not specifically aimed to test LLMs' pragmatic understanding. Given that the understanding of conversational implicature relies heavily on social norms and commonsense knowledge encoded in the Chinese, there is a dire need to investigate whether LLMs possess such knowledge and understanding. 
% spoken language, investigating cross-linguistic pragmatic reasoning in LLMs demonstrates considerable value. 
To address this gap, we select the Chinese sitcom \textit{My Own Swordsman} as the source to formulate pragmatic questions and construct a Chinese dataset for evaluating LLMs' pragmatic reasoning ability.

%In the field of pragmatics, conversational implicature is another instance of going beyond the literal meaning, and understanding sentences with implicature often requires an understanding of the context \citep{yule1996pragmatics}. The cooperative principle is devided into four Gricean Maxims \citep{grice1975logic}, which ask people to be informative (maxim of quantity), truthful (maxim of quality), relevant (maxim of relevance) and clear (maxim of manner) in conversations. Implicature often arises when maxims are violated in utterances. 

%%%Over the past decades, linguists have also studied the characteristics and processes of how people understand implicatures using different approaches.\citep{taguchi2013comprehension,feng2021understanding,jang2013everyday}

%Although today's large language models have strong capabilities in many tasks, they still lag significantly behind humans in understanding implicature \citep{ruis2022large}. Recent studies have examined the pragmatic understanding of the models from different aspects. \citet{qiu2023does} investigated the models' computation of generalized conversational implicatures(GCIs) and found out there is still huge gap between human and models on this task. \citet{kim2023pope} found incorporating Grice's Maxims thorough chain-of-thought prompting can enhance the model ability significantly.  Based on Grice's Maxims, \citet{zheng2021grice} created a dialogue dataset 'GRICE' and evaluated the reasoning ability of the model. \citet{finegrainedPragmatic} later took more complex pragmatic situations into account, including deceit, irony and indirect speech. They also compare the error parttern of both human and the models and found models struggle with phenomena relying on social expectation violents.

%%% As \citet{hancher1980play} states, humor is produced through the violation of speech acts under suitable circumstances or in association with the theory of conversational implicature. \citet{attardo2009linguistic} further discusses the linguistic foundations of humor and the effects of violating Grice's cooperative principle. Recent studies have extracted humorous segments from television sitcoms such as "Friends" and "The Big Bang Theory" and analyzed from the perspective of the Cooperative Principle. \citep{wen2021study,xu2022analysis} In the context of the rapid development of large language models, more analyses of conversational implicatures and the relevant capabilities of LLMs should be conducted.



%%% Table1
\iffalse
\begin{table*}[!ht]
\small
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{p{0.5\textwidth}|p{0.5\textwidth}}
\toprule
\vspace{-96pt}
\begin{tabular}{p{1cm}p{6cm}}
小郭：& 我问你，你是学什么菜系的呀？ \\

大嘴：& 什什么菜系？ \\

小郭：& 川鲁粤淮扬，闽浙湘本帮没听过？ \\

大嘴：& 我手艺是在黄鹤楼学的，黄鹤楼你知道吧。 \\

小郭：& 说句不客气的话，\underline{我进过的酒楼比你上的茅} \underline{房还多}，我尝过的美食比你吃过的饭还多。
\end{tabular}

\vspace{5pt}
\begin{tabular}{p{1.5cm}p{5.5cm}}
Xiaoguo:& So, which Chinese cuisine did you learn? \\

Dazui:& What kind of cuisine? \\

Xiaoguo:& Sichuan, Shandong, Cantonese, Huaiyang. Haven't you heard of local cuisines? \\

Dazui:& I learned my skills at Huanghelou\footnote{A famous Chinese restaurant in ancient China}, you know Huanghelou, right? \\

Xiaoguo:& To be blunt, \ul{I've been to more restaurants than you have been to toilets}, and I've tasted more delicacies than you've eaten meals.
\end{tabular}
&
\begin{tabular}{p{2cm}p{5cm}}
\vspace{5pt}\multirow{2}{*}{\icon{Green}{Pragmatic}} & 小郭想说她自己的见识比大嘴广\\
& Xiaoguo means she's more experienced and knowledgeable than Dazui\\
\hline

\vspace{15pt}\multirow{2}{*}{\icon{Red}{Literal}} & \vspace{3pt} 小郭去过的酒楼的数量比大嘴上过的茅房的数量要多\\
& Xiaoguo has been to more restaurants than Dazui has been to toilets \vspace{1pt}\\

\hline
\vspace{7.5pt}\multirow{2}{*}{\icon{Cerulean}{Distractor\#1}} & \vspace{7.5pt}小郭想去茅房\\
& Xiaoguo wants to go to the toilet\vspace{7.5pt} \\
\hline

\vspace{15pt}\multirow{2}{*}{\icon{Cerulean}{Distractor\#2}} & \vspace{7pt}小郭没听说过黄鹤楼\\
& Xiaoguo haven't heard about Huanghelou\vspace{7pt}
\end{tabular}
\\\bottomrule
\end{tabular}
\end{adjustbox}
\label{tab:eg-in-intro}
\caption{A sample dialogue in our dataset. We offer four interpretations of the underlined sentence that carries a non-literal meaning.}
\end{table*}
\fi
